MicroDiffusion: Implicit Representation-Guided Diffusion for 3D Reconstruction from Limited 2D Microscopy Projections

Volumetric optical microscopy using non-diffracting beams enables rapid imaging of 3D volumes by projecting them axially to 2D images but lacks crucial depth information. Addressing this, we introduce MicroDiffusion, a pioneering tool facilitating high-quality, depth-resolved 3D volume reconstruction from limited 2D projections. While existing Implicit Neural Representation (INR) models often yield incomplete outputs and Denoising Diffusion Probabilistic Models (DDPM) excel at capturing details, our method integrates INR's structural coherence with DDPM's fine-detail enhancement capabilities. We pretrain an INR model to transform 2D axially-projected images into a preliminary 3D volume. This pretrained INR acts as a global prior guiding DDPM's generative process through a linear interpolation between INR outputs and noise inputs. This strategy enriches the diffusion process with structured 3D information, enhancing detail and reducing noise in localized 2D images. By conditioning the diffusion model on the closest 2D projection, MicroDiffusion substantially enhances fidelity in resulting 3D reconstructions, surpassing INR and standard DDPM outputs with unparalleled image quality and structural fidelity. Our code and dataset are available at https://github.com/UCSC-VLAA/MicroDiffusion.

==> sec/cexperiment.tex <==
\section{Experiments}

\subsection{Datasets}
We collected experimental data using a conventional multiphoton laser scanning microscope, which has been a gold standard imaging tool for modern biomedical study. This approach is known for creating a three-dimensional, point-like point spread function. By 3D scanning the tightly focused Gaussian beam, we generated high-quality 3D volume stacks. These stacks serve as ground truth datasets for our research problem. Our setup captures 3D volume stacks of various biological structures—such as dendrites, neurons, and vasculature—within the shallow layers of the mouse cortex in a living animal (Fig.~\ref{fig:definition}). These datasets allow us to test our model with varied 2D projected images from diverse 3D biological features of varying densities.

Subsequently, we generated three synthetic datasets. These datasets simulate the case of fast data acquisition using a non-diffracting beam, whose point spread function has a uniform distribution axially and a predefined width (Fig. 1b). In later experiments, as we will demonstrate, we varied this width to be different multiples (denoted as step length 
$n$) of the point spread function's axial width used to scan and generate the ground truth datasets. Consequently, the acquired 2D image sequences effectively averaged every $n$ frames along the axial direction, with no spatial overlapping in between. This approach reduced the volume data acquisition time by a factor of $n$. We then used both the ground truth and the generated synthetic datasets to evaluate our model at different step length $n$ values, focusing on various datasets from the brain. The design of these datasets allows us to directly determine the optimal step length $n$ value, which will inform both future optimal experimental data acquisition and hardware optical design.

\subsection{Implementation Details}
 Depending on the specific imaging modality, the practical axial width of a non-diffracting beam, such as a Bessel beam, can vary from a few times to tens or hundreds of times that of the point-like Gaussian beam used in conventional 3D laser scanning microscopes \cite{gottschalk2019rapid, chen2018rapid}. We initiate our experiments with a step length \( n \) of approximately 6, which corresponds to roughly an order of magnitude in speed-up — an important initial milestone for volumetric imaging. The performances of different reconstruction models were compared at this setting, and subsequently, an ablation study was conducted over the step length value. This study aims to further understand the impact of the step length of \( n \) on reconstruction quality, with the goal of identifying the optimal trade-off region between \( n \) times speed-up and image reconstruction quality.
  
 For computational efficiency, we downsample all the samples to a resolution of \( 128 \times 128 \) pixels in the lateral plane. For the pure Implicit Neural Representation (INR) model and the INR encoder, we map the 3D coordinates to a 512-dimensional space using a Gaussian-based embedding technique. The INR model is optimized using the Adam optimizer with a learning rate of \( 10^{-3} \) over 5000 epochs, a process that takes approximately 8 hours on an A-100 GPU. Additionally, we employ the AdamW optimizer with a learning rate of \( 2^{-4} \) and a weight decay of \( 10^{-4} \). As for the diffusion model, it is trained over 2000 epochs, taking around 4 hours on a single NVIDIA A-100 GPU.


\subsection{Baselines}
Given the novelty of this task and the absence of existing reference works, we established  baseline methods. The initial approach is a straightforward \textit{Interpolation} method, in which the generated structure is created through a uniformly weighted average of the two adjacent projections, weighted according to their distance. And \textit{Interpolation - cubic}, which estimates values by using cubic polynomials between points. This means that each interpolated curve segment is based on the position and slope (derivative) at its endpoints. The last baseline employs a pure INR method, which functions as our prior to the diffusion model.

\subsection{Reconstruction Results}


\subsubsection{Quantitative Results}             We evaluate our methods using three metrics: Peak Signal-to-Noise Ratio (PSNR), Structural Similarity Index Measure (SSIM), and the Dice coefficient. PSNR and SSIM are calculated slice-wise along the axial direction, with the mean value across all slices being reported. For the DICE coefficient, we  use the OTSU~\cite{otsu1979threshold} algorithm to determine the threshold for each image to assess the volumetric similarity between the generated 3D structure and the ground truth.
As presented in Table \ref{tab:main_result}, our method demonstrates strong performance, successfully capturing the principal structure of the original high-resolution model. Additionally, we observe that the diffusion model's decoder significantly enhances the performance of the pure INR model. %This improvement is particularly notable in the beads datasets, which are sparser compared to the other datasets.     

\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{c|c|ccc}
   \toprule
   Dataset & Method & SSIM $\uparrow$ & PSNR $\uparrow$ & DICE $\uparrow$ \\
   \midrule
   \multirow{3}{*}{Dendrite} 
   &Interpolation         & 0.9696             & 28.78 & 0.6482 \\ 
   &Interpolation - cubic  & 0.9770 & 28.85 & 0.3973 \\ 
   &INR & 0.6262 & 25.81 & 0.4589   \\ 
   % &MicroDiffusion - join         & - & - & -  \\   
   &MicroDiffusion  & \textbf{0.8409} & \textbf{29.74} & \textbf{0.7557}  \\ 
   \midrule
    \multirow{3}{*}{Vasculature} 
   &Interpolation        & 0.9445             & 20.42 & 0.5936 \\ 
   &Interpolation - cubic  & 0.9586 & 20.52 & 0.4448 \\
   &INR                    & 0.7898 & 21.69 & 0.7136 \\  
   % &MicroDiffusion - join         & - & - & -  \\   
   &MicroDiffusion       & \textbf{0.8376} & \textbf{22.35} & \textbf{0.7158}  \\   
   \midrule
   \multirow{3}{*}{Neuron} 
   &Interpolation         & 0.8385  & 24.12 & 0.3553 \\ 
   &Interpolation - cubic  & 0.8770 & 26.50 & 0.1116 \\ 
   &INR                    & 0.9135 & 26.43 & 0.6403 \\
   &MicroDiffusion       & \textbf{0.6009} & \textbf{26.66} & \textbf{0.6708} \\   
   \bottomrule
\end{tabular}
\caption{Main results of the image reconstruction quality across different datasets with different biological features: vasculature, neurons, and dendrites. For all metrics, higher values indicating better performance as indicated by the arrows. The best results in each category are highlighted in bold.}
\label{tab:main_result}
\end{table}

                 



% \begin{table}[!t]
%     \centering
%     \caption{Experiment results on the \but{dataset name} dataset}
%     \begin{tabular}{lcccc}
    
%         \but{dataset name} & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$  \\ \toprule
%         INR & 0.9286 & 21.69 & 0.7136  \\ \hline
%         MicroDiffusion & 0.9822 & 22.35 & 0.7158  \\ 
%         \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[!t]
%     \centering
%         \caption{Experiment results on the beads dataset}
%     \begin{tabular}{lcccc}
%     \toprule
%         beads & SSIM $\uparrow$ & PSNR $\uparrow$ & DICE $\uparrow$  \\ \hline
%         INR & 0.5425 & 15.77 & 0.7045  \\ \hline
%         MicroDiffusion & 0.8138 & 20.31 & 0.7325  \\ 
%         \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[!t]
%     \centering
%         \caption{Experiment results on the YFP dataset}
%     \begin{tabular}{lcccc}
%     \toprule
%         beads & SSIM $\uparrow$ & PSNR $\uparrow$ & DICE $\uparrow$  \\ \hline
%         INR & 0.9768 & 25.81 & 0.7045  \\ \hline
%         MicroDiffusion & 0.9848 & 29.74 & 0.7325  \\ 
%         \bottomrule
%     \end{tabular}
% \end{table}



\subsubsection{Qualitative Results}
Here, we present the reconstruction results of three methods: pure INR and MicroDiffusion. Part of the slices from the reconstructed 3D stacks are illustrated in Fig. \ref{fig:sampling_slices}, where we randomly selected three slices from the 3D reconstructions generated by naive diffusion, the pure INR reconstruction, our MicroDiffusion and compare with ground truth.  From these results, it is evident that the reconstructions obtained via the MicroDiffusion method more closely resemble the ground truth as the density of the biological features increases. This result indicates an encouraging possibility that volumetric imaging with a non-diffracting beam allows not only well-known volumetric imaging of sparse features such as neurons in the cortex \cite{chen2018rapid} but also denser features such as vasculature  and even dense dendrites.
\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{fig/PanelFigure2.pdf}
    % \vspace{-6mm}
    \caption{Qualitative results: (a) Comparative visualization of slices from 3D reconstructions with different methods. Observable differences between the INR reconstruction, MicroDiffusion reconstruction, and ground truth are indicated with white arrows. (b) 3D vasculature. Scale bar: 30 $\mu$m.}
\label{fig:sampling_slices}
\vspace{-6mm}
\end{figure}

\subsection{Ablation study}
\subsubsection{Ablation on conditional feature}
\paragraph{How to encode 3D positional information}
We initially evaluate two positional encoding methods for MicroDiffusion: (1) the sine-cosine based encoding as described by NeRF \cite{mildenhall2020nerf}, and (2) the Gaussian-based encoding used in NeRP \cite{shen2023nerp}. As shown in Table \ref{tab:position_ablation}, our experiment results demonstrate that the Gaussian-based encoding yields superior results, particularly in rendering clearer textures. We attribute this improvement to the intrinsic properties of Gaussian embeddings, which affords a more flexible mapping of positions to a higher-dimensional space. This flexibility enhances the subsequent learning process within MicroDiffusion, leading to more detailed and accurate representations.
\begin{table}[htbp]
\vspace{-3mm}
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule
        Method & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
    \midrule
        Sin-cos &  0.9449& 21.03& 0.6667\\ 
        gassian-based(ours) & \textbf{0.9822} & \textbf{22.35} & \textbf{0.7158} \\  
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation of the positional encoding type on vasculature. }
    \label{tab:position_ablation}
\end{table}
\vspace{-8mm}
\paragraph{How to add conditional feature }
We ablate on the way we incorporate the conditional feature $c$ into the model. \textit{w/o feature guidance} involves setting all conditions to $\emptyset$. \textit{cross-attention} involves adding $c$ using cross-attention to replace the self-attention in Denoising U-net, where the image feature is the query, and the conditional feature $c$ serves as the key and value. Experimental results demonstrate that adding the conditional feature $c$ is effective and leads to the best performance. This is likely because we have only one conditional feature, and in such a case, the cross-attention mechanism may not be effective. Therefore, it is better to directly add the conditional feature to the output of each ResNet block in the Denoising U-net.
\vspace{-3mm}
\begin{table}[htbp]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
         method & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
        \midrule
        w/o feature guidance & 0.9474 & 21.27 & 0.6512  \\ 
        cross-attention & 0.9733 & 21.25 & 0.6784 \\
         addition (ours) & \textbf{0.9822} & \textbf{22.35} & \textbf{0.7158} \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation results fusion ablation on vasculature}
    \label{tab:fusion_ablation}
\end{table}
\vspace{-3mm}

\subsubsection{Ablation on INR prior}
\paragraph{How to generate INR prior?}
Here, we test three INR prior generation methods as shown in Table \ref{tab:neighbour_ablation}. \textit{no-neighbouring} means that we only utilize the INR output corresponding to the current 3D coordinate $z$ as the INR prior.
\textit{uniformly-mean} means that we use the uniformly averaged output of the INR corresponding to the six frames centered on the current 3D coordinate $z$.
The experimental results demonstrate that our approach performs the best when introducing Neighbouring-based Inference, allowing the model to obtain a more comprehensive 3D INR prior.


\begin{table}[htbp]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule
        method & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
    \midrule
        no-neighbouring  & 0.8359& 15.26& 0.2025\\   
        uniformly-mean  & 0.9126 & 17.36 & 0.4086 \\ 
        Neighbouring-based (ours)  & \textbf{0.9822} & \textbf{22.35} & \textbf{0.7158} \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation of neighbouring based inference on vasculature.}
    \label{tab:neighbour_ablation}
\end{table}
\vspace{-3mm}

\paragraph{How to add INR prior?} 
We investigate the necessity of the INR prior in this experiment. We trained a naive diffusion model that incorporates the INR prior as the projection introduced in~\ref{par:snap}.
We use the image encoder $E_{img}$ to encode the output of INR $m_{inr}$ and concatenate the feature with the other conditions.
This allows the model to generate images that resemble true biological features. However, this method performs poorly in acquiring global information, as evidenced by the very low DICE result in Table \ref{tab:prior_ablation}. 

% \vspace{-2mm}
\begin{table}[htbp]
    \centering
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{l|ccc}
    \toprule
        Method & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
    \midrule
        Naive Diffusion &  0.8916& 14.97& 0.4540\\ 
        MicroDiffusion & \textbf{0.9822} & \textbf{22.35} & \textbf{0.7158} \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation of diffusion model INR prior on the vasculature.}
    \label{tab:prior_ablation}
\end{table}

\vspace{-4mm}
\subsubsection{Ablation on training method}
\vspace{-1mm}
In our pipeline, we adopt a two-stage training process where the INR is trained initially and then frozen during the MicroDiffusion training. We conducted ablation experiments to explore two alternatives: (1) \textit{joint-training}, where we jointly train INR and the Denoising U-Net from random initialization, and (2) \textit{trainable}, where we unfreeze the INR during the MicroDiffusion training.

We used the same number of epochs for all methods. For \textit{joint-training}, we added the INR loss and applied a decaying weight to balance the training dynamics. As shown in Table \ref{tab:joint_ablation}, our method achieved the best performance. However, \textit{joint-training} proved to be too challenging and adversely affected the MicroDiffusion training process, while \textit{trainable} impaired the ability of INR to provide priors.

Therefore, we chose to train INR first and then train MicroDiffusion with it frozen.

 % \hongru{[What do we want to say here?]}
\begin{table}[htbp]
% \vspace{-2mm}
    \centering
        \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
         method & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
        \midrule
        joint-training & 0.9691 & 21.37 & 0.6603 \\
        trainable & 0.7909 & 21.27 & 0.6875  \\ 
        freeze (ours) & \textbf{0.8376} & \textbf{22.35} & \textbf{0.7158}  \\
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation results of training methold on vasculature}
    \label{tab:joint_ablation}
\end{table}

\vspace{-8mm}
    
\subsubsection{Ablation on Different Step length}

We investigate the impact of the step length on MicroDiffusion performance. As outlined in our methodology, a larger step size results in faster volumetric imaging but makes reconstruction more challenging. Conversely, smaller step size leads to slower imaging but improved reconstruction. We keep the number of iterations the same and train our model from scratch. Results are presented in Figure \ref{fig:metrics}.

We observed that as the step length increased, all model metrics gradually decreased. To strike a reasonable balance between sampling speed and reconstruction quality, we chose a step length of 6.

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{cc|ccc}
%     \toprule
%         Step length $n$ & SSIM$\uparrow$ & PSNR$\uparrow$ & DICE$\uparrow$ \\ 
%     \midrule
%         4 &0.9894 & 24.31 & 0.8030 \\
%         6(ours) &0.9822 & 22.35 & 0.7158 \\  
%         8 &0.9801 & 21.91 & 0.6726\\
%         16 &0.9538 & 17.72 & 0.4259\\
%         32 &0.9266 & 15.70 & 0.2623\\
%         65 &0.9274 & 14.95 & 0.2030\\
%         130 &- & - & -\\
%     \bottomrule
%     \end{tabular}
%     \caption{Ablation of the step size on the vasculature. }
%     \label{tab: step_ablation}
% \end{table}

\begin{figure}[h]
\vspace{-3mm}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{fig/combined_graph.pdf}
        \caption{SSIM, PSNR and DICE}
        \label{fig:dice}
    \end{subfigure}
    \caption{Performance metrics across different step lengths.}
    \label{fig:metrics}
\end{figure}
 \vspace{-3mm}
 
\subsection{Discussion and Future Work}
In our experiments, we find that when ground truth data contains Gaussian noise, MicroDiffusion outperforms other methods in noise removal. This demonstrates the potential of MicroDiffusion for denoising 3D volumes acquired by volumetric optical microscopy. In cases where Gaussian noise is intentionally part of the Ground Truth data and should not be removed, it is necessary to investigate how to use other types of noise for MicroDiffusion training.
